An Intelligent Self-driving Truck System For Highway Transportation

Recently, there have been many advances in autonomous driving society, attracting a lot of attention from academia and industry. However, existing works mainly focus on cars, extra development is still required for self-driving truck algorithms and models. In this paper, we introduce an intelligent self-driving truck system. Our presented system consists of three main components, 1) a realistic traffic simulation module for generating realistic traffic flow in testing scenarios, 2) a high-fidelity truck model which is designed and evaluated for mimicking real truck response in real-world deployment, 3) an intelligent planning module with learning-based decision making algorithm and multi-mode trajectory planner, taking into account the truck's constraints, road slope changes, and the surrounding traffic flow. We provide quantitative evaluations for each component individually to demonstrate the fidelity and performance of each part. We also deploy our proposed system on a real truck and conduct real world experiments which shows our system's capacity of mitigating sim-to-real gap. Our code is available at https://github.com/InceptioResearch/IITS

==> exp-bak.tex <==


\section{Experiment Setup}

\subsection{Platform Fidelity Validation}

We build our RL model based on Pytorch~\cite{paszke2019pytorch} and train it on a ThinkStation P920 with Intel Xeon(R) Silver 4110 2.1GHz x32 and NVIDIA RTX 2080Ti. During the training process, the learning rate is fixed as $5\mathrm{e}{-4}$, the optimizer is ADAM~\cite{kingma2014adam}, and the training batch size sets as $32$. Our simulation platform is running at \SI{10}{Hz}. Note that up to six cars in front of the ego-truck and two cars behind the ego-truck are observable. The model is trained for $2$ days, and the reward curve is shown in~\prettyref{fig:rewardcurve}.


\begin{figure}[htbp] 
	\centering
    \begin{subfigure}[b]{1.0\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/val1.png}
        \caption[Network2]%
        {{\small Gear Position}}    
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{1.0\linewidth}  
        \centering 
        \includegraphics[width=\linewidth]{fig/val2.png}
        \caption[]%
        {{\small Velocity}}    
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{1.0\linewidth}  
        \centering 
        \includegraphics[width=\linewidth]{fig/val3.png}
        \caption[]%
        {{\small Acceleration}}    
    \end{subfigure}
	\caption{\label{fig:verlong}%
		Results of the experiments on verifying the accuracy of the truck model. Red lines indicate simulated results, and blue lines are real data from the truck. The results demonstrate that our truck model is highly close to the real truck.
	}
	%\vspace{-0.5cm}
\end{figure} 

\begin{figure}[htbp] 
	\centering
	\mbox{} \hfill
	\includegraphics[ width=1\linewidth]{fig/rewardCurve.png}
	\hfill \mbox{}
	\caption{\label{fig:rewardcurve}%
		Average accumulative reward for each epoch during the training procedure.
	}
	%\vspace{-0.5cm}
\end{figure} 

\begin{table*}[!h]
\centering
\resizebox{0.8\textwidth}{!}{  
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Scenario                & Traffic Speed & Conservative-BSL & Neutral-BSL & Aggressive-BSL & Ours \\ \hline
\multirow{3}{*}{Dense}  & 10m/s         &  40.079\%/0.061  &  38.597\%/0.059  & \textbf{30.900\%}/0.047  & 33.872\%/0.052 \\ \cline{2-6} 
                        & 12.5m/s       &  38.900\%/0.059 &  28.503\%/0.043  & 24.530\%/0.038 & \textbf{24.032\%}/0.037 \\ \cline{2-6} 
                        & 15m/s         &  30.889\%/0.047 &  20.125\%/0.031  & 18.773\%/0.028 & \textbf{17.331\%}/0.027 \\ \hline
\multirow{3}{*}{Medium} & 10m/s         &  22.122\%/0.034  &  17.805\%/0.027& \textbf{11.571\%}/0.018 &  15.073\%/0.023 \\ \cline{2-6} 
                        & 12.5m/s       &  14.087\%/0.022   &   13.766\%/0.021 & \textbf{6.592\%}/0.010  & 7.969\%/0.012 \\ \cline{2-6} 
                        & 15m/s         &  4.425\%/0.007  &  1.591\%/0.002  &  1.549\%/0.002  & \textbf{1.399\%}/0.002 \\ \hline
\multirow{3}{*}{Sparse} & 10m/s         &  13.102\%/0.020   & 9.996\%/0.015  &   \textbf{3.429\%}/0.005  &  3.877\%/0.006 \\ \cline{2-6} 
                        & 12.5m/s       &  5.894\%/0.009 &  3.425\%/0.005   & 4.396\%/0.007   & \textbf{3.393\%}/0.005 \\ \cline{2-6} 
                        & 15m/s         & 1.005\%/0.001  & 0.998\%/0.001   &  0.998\%/0.002  & \textbf{0.998\%}/0.001 \\ \hline
\end{tabular}
}
\caption{Average Delta Velocity (shown as mean/std) evaluated for different methods on different scenarios, and the best results in each category are in \textbf{bold}. Note that Conservative-BSL in table is the abbreviation of the conservative baseline.
} 
\label{tab:delta_t} 
\end{table*}

\begin{table*}[!h]
\centering
\resizebox{0.75\textwidth}{!}{  
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Scenario                & Traffic Speed & Conservative-BSL & Neutral-BSL & Aggressive-BSL & Ours \\ \hline
\multirow{3}{*}{Dense}  & 10m/s         &  1.59/1.42  &  6.00/2.61  &  6.13/2.65   & \textbf{5.89}/2.58 \\ \cline{2-6} 
                        & 12.5m/s       &  2.84/1.76   &  6.23/2.67    & 6.98/3.87  & \textbf{6.16}/2.65 \\ \cline{2-6} 
                        & 15m/s         &  3.06/1.82   &  6.89/2.85    &  7.13/3.91   & \textbf{6.24}/2.68  \\ \hline
\multirow{3}{*}{Medium} & 10m/s         &  4.29/1.15    &  5.66/2.53    & 7.32/3.52     & \textbf{6.98}/2.87 \\ \cline{2-6} 
                        & 12.5m/s       &  4.58/1.23    & 5.09/2.37    &  8.93/3.39    &  \textbf{6.22}/2.67 \\ \cline{2-6} 
                        & 15m/s         &  5.00/1.34  & 4.02/2.08   &  8.99/3.41    & \textbf{6.30}/2.69 \\ \hline
\multirow{3}{*}{Sparse} & 10m/s         &  2.03/1.55  & 2.03/1.54     &  2.88/1.77    & \textbf{2.52}/1.68  \\ \cline{2-6} 
                        & 12.5m/s       &  2.55/0.68    & 2.83/0.75   &  2.99/0.80    & \textbf{3.02}/0.81 \\ \cline{2-6} 
                        & 15m/s         & 0.40/0.11    & 0.40/0.10    & 0.50/0.13    & 0.77/0.21  \\ \hline
\end{tabular}
}
\caption{Average Count of Lane Change (shown as mean/std) evaluated for different methods on different scenarios. Since we achieve a comparable result on delta velocity comparing with aggressive baseline, we high-light our number in bold if our method conducts fewer change than the aggressive baseline.} 
\label{tab:lccount}
%%\vspace{-0.5cm}
\end{table*}

\section{Numerical Simulation Experiments}
In this section, we illustrate the verification experiments of our truck model firstly. Then, we introduce the performance metric and test scenarios for evaluation. After that we compare our method with other methods and demonstrate the quantitative and qualitative results. Finally, we discuss the result and performance.

\subsection{Performance Metrics and Test Scenarios}
For performance comparison between our approach and other methods, we present the following metrics for quantitative evaluation:
\begin{enumerate}
\item Delta Velocity: the average difference between ego-truck speed $V$ and reference speed $V_{ref}$. It is formulated as: $\nabla V = (V_{ref} - V)/V_{ref}$.
\item Count of Lane Change: the average count of lane change decision during the journey.
\end{enumerate}

In order to demonstrate the capability of dealing with different densities and character of traffic, we investigate traffic with three different densities and three average speeds in our experiment.

For the density aspect, we modify the spawn probability as $0.05$, $0.02$, $0.005$, corresponding to the dense, medium, sparse density respectively. For the average speed of traffic aspect, we set the maximum speed of the traffic flow as \SI{10}{m/s}, \SI{12.5}{m/s}, \SI{15}{m/s}, and our ego-truck's reference speed is fixed as \SI{16.67}{m/s} (\SI{60}{km/h}) which is suitable for most logistics operations. 

For comparison, we propose three baseline algorithms with rule-based FSM to mimic different characteristic drivers' behavior, which is widely used in industry. When the ego-truck detects obstacles $d$\si{m} ahead of it, we will check whether there is no traffic in the neighbor lane with $d$\si{m} ahead of it and $d$\si{m} back of it. If so, the lane change decision will be sent to the trajectory planner; if not, we will keep in this lane. Here, we use $d$ to describe the drivers' characteristics: aggressive, neutral and conservative, corresponding to $d=50, 100$ and $150$, as shown in~\prettyref{tab:delta_t} and~\prettyref{tab:lccount}.

\subsection{Comparison and Discussion}
\begin{figure*}[htbp] 
	\centering
    \begin{subfigure}[b]{0.33\linewidth}
        \centering
        \includegraphics[width=\linewidth]{fig/dense_plot.png}
        \caption[Network2]%
        {{\small dense}}    
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}  
        \centering 
        \includegraphics[width=\linewidth]{fig/medium_plot.png}
        \caption[]%
        {{\small medium}}    
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.31\linewidth}  
        \centering 
        \includegraphics[width=\linewidth]{fig/sparse_plot.png}
        \caption[]%
        {{\small sparse}}    
    \end{subfigure}
	\caption{\label{fig:resultplot}%
		Experiment results. $x$ axis represents the lane change count in~\prettyref{tab:lccount}, and $y$ axis represents the delta velocity in~\prettyref{tab:delta_t}. The red, green and blue lines represent traffic with a max speed of \SI{10}{m/s}, \SI{12.5}{m/s} and \SI{15}{m/s}, respectively. The triangle, rhombus, circle and star signs denote the conservative baseline, the neutral baseline, the aggressive baseline and our RL method, respectively. Since our goal is to achieve the reference speed (lower delta velocity) with as few lane changes as possible (lower lane change count) while ensuring safety, the method closer to the origin is better.
	}
	%%\vspace{-0.5cm}
\end{figure*} 

We compare our RL based lane change decision-maker with aggressive, neutral and conservative baseline algorithms. Note that except the decision-maker module, all other modules remain unchanged. We run each experiment trial $30$ times and compute the mean value of them.

~\prettyref{tab:delta_t} and~\prettyref{tab:lccount} show the performance evaluated using different methods in different test scenarios. In~\prettyref{tab:delta_t}, it can be seen that our RL base method yields the best performance according to delta velocity metrics in most cases. We noticed that our method's performance is worse than the aggressive baseline algorithm. This is because that aggressive baseline tends to change lane frequently. Ideally, if the ego-truck can change the lane frequently enough that the influence of any car in front of it can be avoided. However, because of the character of the truck we mentioned in the introduction section, it is impossible, even dangerous, for a truck to be tap-dancing through the traffic flow. That is the reason why we add a penalty for all lane change decisions in our reward function for the RL. Our goal is to achieve the reference speed with as few lane changes as possible while ensuring safety. In~\prettyref{tab:lccount}, we can observe that our RL based approach changes lane fewer than the aggressive baseline algorithm in most cases. With fewer change, we also achieve comparable performance compared to baseline methods. 

To illustrate the trade-off between lane change times and delta velocity performance, we plot the experiment result in~\prettyref{fig:resultplot}, where $x$ axis represents the lane change count in~\prettyref{tab:lccount}, and $y$ axis represents the delta velocity in~\prettyref{tab:delta_t}. From left to right, we have three subplots, which represent dense scenarios, medium scenarios and sparse scenarios respectively. In each subplot, we use red lines and signs to represent \SI{10}{m/s} traffic scenario cases, green lines and signs as \SI{12.5}{m/s} traffic flow, then blue lines and signs are the traffic with a max speed of \SI{15}{m/s}. Moreover, the triangle, rhombus, circle and star signs represent the conservative baseline, the neutral baseline, the aggressive baseline, and our RL method, respectively.

Since our goal is to achieve the reference speed with as few lane changes as possible, the method that is closer to the origin is better. In~\prettyref{fig:resultplot} (c), most of the signs are clustered together, especially the green case (\SI{12.5}{m/s}) and blue case (\SI{15}{m/s}). The reason is the traffic is too sparse in these experiments and thus each methods' performance are very close. But in red experiments (\SI{10}{m/s} sparse traffic), our method is located at the bottom of the red line and closest to the origin, which means our method performs best in this scenario comparing to all baseline methods. In~\prettyref{fig:resultplot} (b), we can observe that although delta velocity of our method in the green experiment (\SI{12.5}{m/s}, medium) is lower than the aggressive baseline, but our point is closest to the origin, which means we use fewer change to achieve comparable performance. In~\prettyref{fig:resultplot} (a), obviously our method performs the best, almost all star signs are under the line.

\section{Real Truck Validation}
\subsection{Validation of Truck Model}
\label{sec:val_truckmodel}
To verify the accuracy of our truck model, we collect some data from a real truck running with a human driver, then replay the truck control commands in our simulator and compare the difference in vehicle response. We illustrate one of results in~\prettyref{fig:verlong}, where the red lines indicate the simulated results and the blue lines are the real data from trucks. We can observe that the blue and red lines almost coincide with each other. The mean velocity accuracy of all experiments is 89\% and the yaw rate steady accuracy is 92\%. These experiments verify that our truck model is highly close to the real truck. 

\subsection{Real Truck Experiment in Closed Test Site}
TO BE Done


==> exp.tex <==

\section{Experimental results}

In this section, we illustrate the verification experiments of platform fidelity firstly. Then, we show the experiment of the RL baseline training on our platform. Finally, we migrate our platform along with trained RL model to the real truck.

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.475\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{fig/jinan_real.png}
%         \caption[]%
%         {{\small Simulation Experiment}}    
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.475\linewidth}  
%         \centering 
%         \includegraphics[width=\linewidth]{fig/jinan_virtual.png}
%         \caption[]%
%         {{\small Real Truck Test}}    
%     \end{subfigure}
%     \caption
%     {\small We migrate our RL baseline to real truck and arrange the same test scenarios in Jinan.}
%     \label{fig:sensor_simulation}
% \end{figure}

\subsection{Platform Validation}
In order to validate our platform, we evaluate two simulation modules: Truck Model and Traffic Simulation. Since the Sensor Simulation module relies on the open sourced simulator CARLA, it is unnecessary for us to evaluate this part. 

\subsubsection{Traffic flow}
The traffic simulation node is implemented with SUMO. We can support not only the maps created by hands, but also the HD map of the real road networks (see ~\prettyref{fig:maps}). With the diverse maps as the environments, we can generate various traffic flows.  

Our traffic simulation node can generate similar traffic with the real-world datasets. We compare the velocity distributions with those of the real-world datasets. We choose three datasets with different traffic flow densities (sparse, middle and dense). The velocity distributions with different traffic densities are shown in~\prettyref{fig:vel_distri}. Our results are close to those of the real-world datasets.

\begin{figure}[!h] 
	\centering
    % \includegraphics[width=\linewidth]{fig/exp-steering-system.png}
        \includegraphics[width=\linewidth]{fig/exp-steering-system.pdf}
	\caption{\label{fig:exp-steering-system}%
		Steering system experiments. Red lines indicate simulated results, and blue lines are real data from the truck. The results demonstrate that our TruckSim lateral model is highly close to the real truck.
	}
	\vspace{-0.5cm}
\end{figure} 

\subsubsection{Fidelity of Longitudinal Model}
To verify the accuracy of the longitudinal model, we collect some data from a real truck running with a human driver, then replay the truck control commands in our simulator and compare the difference in vehicle response. ~\prettyref{fig:driveline} shows results of the experiments on verifying the drive-line and brake subsystems, with Fig.~\ref{subfig:driveline_a} and Fig.~\ref{subfig:driveline_b} corresponding to the truck's acceleration and brake motions respectively, where the red lines indicate the simulated results and the blue lines are the real data from trucks. The results validate that the behavior of our truck model is highly close to the real truck.


\subsubsection{Fidelity of Lateral TruckSim Model}
TruckSim model in ATS is used to describe the lateral motion of the truck. It combines steering system, solid axles and tire system together so that the physical characteristics of the real truck can be restored to the utmost extent. Same as the evaluation experiment of longitudinal model, we replay the control commands in our simulator and compare the responses. Results in~\prettyref{fig:exp-steering-system} verify that the TruckSim's lateral performance is highly close to the real truck.

\begin{figure}[!h] 
	\centering
    \includegraphics[width=\linewidth]{fig/step_comb.pdf}
	\caption{\label{fig:step_comb}%
		Results of the experiments on verifying the accuracy of the dynamic yaw-sideslip model. Red lines indicate results of alternative model, and blue lines are data from TruckSim model. The results demonstrate that our dynamic yaw-sideslip model is highly close to TruckSim model.
	}
	\vspace{-0.5cm}
\end{figure} 

\subsubsection{Fidelity of Dynamic Yaw-sideslip Model}
The dynamic yaw-sideslip model is designed as an alternative choice of TruckSim model, thus we conduct an experiment to compare the dynamic yaw-sideslip model with the TruckSim lateral model. During the comparison experiment, we set the truck speed at \SI{80}{km/h} and we fed a step steering command of 15 degrees to each model. Results are shown in~\prettyref{fig:step_comb}, where the red line indicates the response of dynamic yaw-sideslip model and blue line refers to the result of TruckSim model. The result demonstrate that our dynamic yaw-sideslip model is highly close to TruckSim model, whose accuracy is enough for replace TruckSim model in our platform. 
  

% The truck drives at speed of 80 km/h and a step steering command of 15 degree is fed to each model. 

% \begin{figure}[!h] 
% 	\centering
%     \begin{subfigure}[b]{1.0\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{fig/val1.png}
%         \caption[Network2]%
%         {{\small Gear Position}}    
%     \end{subfigure}
%     \vskip\baselineskip
%     \begin{subfigure}[b]{1.0\linewidth}  
%         \centering 
%         \includegraphics[width=\linewidth]{fig/val2.png}
%         \caption[]%
%         {{\small Velocity}}    
%     \end{subfigure}
%     \vskip\baselineskip
%     \begin{subfigure}[b]{1.0\linewidth}  
%         \centering 
%         \includegraphics[width=\linewidth]{fig/val3.png}
%         \caption[]%
%         {{\small Acceleration}}    
%     \end{subfigure}
% 	\caption{\label{fig:verlong}%
% 		Results of the experiments on verifying the accuracy of the truck model. Red lines indicate simulated results, and blue lines are real data from the truck. The results demonstrate that our truck model is highly close to the real truck.
% 	}
% 	%\vspace{-0.5cm}
% \end{figure} 

% \begin{figure}[!h] 
% 	\centering
% 	\mbox{} \hfill
% 	\includegraphics[ width=1\linewidth]{fig/rewardCurve.png}
% 	\hfill \mbox{}
% 	\caption{\label{fig:rewardcurve}%
% 		Average accumulative reward for each epoch during the training procedure.
% 	}
% 	%\vspace{-0.5cm}
% \end{figure} 

% \subsection{Performance Metrics and Test Scenarios}


% To illustrate the trade-off between lane change times and delta velocity performance, we plot the experiment result in~\prettyref{fig:resultplot}, where $x$ axis represents the lane change count in~\prettyref{tab:lccount}, and $y$ axis represents the delta velocity in~\prettyref{tab:delta_t}. From left to right, we have three subplots, which represent dense scenarios, medium scenarios and sparse scenarios respectively. In each subplot, we use red lines and signs to represent \SI{10}{m/s} traffic scenario cases, green lines and signs as \SI{12.5}{m/s} traffic flow, then blue lines and signs are the traffic with a max speed of \SI{15}{m/s}. Moreover, the triangle, rhombus, circle and star signs represent the conservative baseline, the neutral baseline, the aggressive baseline, and our RL method, respectively.

% Since our goal is to achieve the reference speed with as few lane changes as possible, the method that is closer to the origin is better. In~\prettyref{fig:resultplot} (c), most of the signs are clustered together, especially the green case (\SI{12.5}{m/s}) and blue case (\SI{15}{m/s}). The reason is the traffic is too sparse in these experiments and thus each methods' performance are very close. But in red experiments (\SI{10}{m/s} sparse traffic), our method is located at the bottom of the red line and closest to the origin, which means our method performs best in this scenario comparing to all baseline methods. In~\prettyref{fig:resultplot} (b), we can observe that although delta velocity of our method in the green experiment (\SI{12.5}{m/s}, medium) is lower than the aggressive baseline, but our point is closest to the origin, which means we use fewer change to achieve comparable performance. In~\prettyref{fig:resultplot} (a), obviously our method performs the best, almost all star signs are under the line.

% \section{Real Truck Validation}


% \subsection{Real Truck Experiment in Closed Test Site}
% TO BE Done

